Submillimetre observations of WISE-selected high-redshift, luminous, dusty galaxies

We present SCUBA-2 850um submillimetre (submm) observations of the fields of 10 dusty, luminous galaxies at z ~ 1.7 - 4.6, detected at 12um and/or 22um by the WISE all-sky survey, but faint or undetected at 3.4um and 4.6um; dubbed hot, dust-obscured galaxies (Hot DOGs). The six detected targets all have total infrared luminosities greater than 10^13 L_sun, with one greater than 10^14 L_sun. Their spectral energy distributions (SEDs) are very blue from mid-infrared to submm wavelengths and not well fitted by standard AGN SED templates, without adding extra dust extinction to fit the WISE 3.4um and 4.6um data. The SCUBA-2 850um observations confirm that the Hot DOGs have less cold and/or more warm dust emission than standard AGN templates, and limit an underlying extended spiral or ULIRG-type galaxy to contribute less than about 2% or 55% of the typical total Hot DOG IR luminosity, respectively. The two most distant and luminous targets have similar observed submm to mid-infrared ratios to the rest, and thus appear to have even hotter SEDs. The number of serendipitous submm galaxies (SMGs) detected in the 1.5-arcmin-radius SCUBA-2 850um maps indicates there is a significant over-density of serendipitous sources around Hot DOGs. These submm observations confirm that the WISE-selected ultra-luminous galaxies have very blue mid-infrared to submm SEDs, suggesting that they contain very powerful AGN, and are apparently located in unusual arcmin-scale overdensities of very luminous dusty galaxies.

==> aas_abbrev.tex <==
\newcommand\aj{AJ}%
          % Astronomical Journal
\newcommand\actaa{Acta Astron.}%
 	  % Acta Astronomica
\newcommand\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{ApJ}%
          % Astrophysical Journal
\newcommand\apjl{ApJ}%
          % Astrophysical Journal, Letters
\newcommand\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\newcommand\ao{Appl.~Opt.}%
          % Applied Optics
\newcommand\apss{Ap\&SS}%
          % Astrophysics and Space Science
\newcommand\aap{A\&A}%
          % Astronomy and Astrophysics
\newcommand\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{AZh}%
          % Astronomicheskii Zhurnal
\newcommand\baas{BAAS}%
          % Bulletin of the AAS
\newcommand\caa{Chinese Astron. Astrophys.}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{Chinese J. Astron. Astrophys.}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{Icarus}%
  % Icarus
\newcommand\jcap{J. Cosmology Astropart. Phys.}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{JRASC}%
          % Journal of the RAS of Canada
\newcommand\memras{MmRAS}%
          % Memoirs of the RAS
\newcommand\mnras{MNRAS}%
          % Monthly Notices of the RAS
\newcommand\na{New A}%
  % New Astronomy
\newcommand\nar{New A Rev.}%
  % New Astronomy Review
\newcommand\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\newcommand\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\newcommand\prc{Phys.~Rev.~C}%
          % Physical Review C
\newcommand\prd{Phys.~Rev.~D}%
          % Physical Review D
\newcommand\pre{Phys.~Rev.~E}%
          % Physical Review E
\newcommand\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\newcommand\pasa{PASA}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{PASP}%
          % Publications of the ASP
\newcommand\pasj{PASJ}%
          % Publications of the ASJ
\newcommand\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{Rev. Mexicana Astron. Astrofis.}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{S\&T}%
          % Sky and Telescope
\newcommand\solphys{Sol.~Phys.}%
          % Solar Physics
\newcommand\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\newcommand\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\newcommand\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{Nature}%
          % Nature
\newcommand\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\newcommand\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters and Communications
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\newcommand\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\newcommand\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\newcommand\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\newcommand\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysical Research
\newcommand\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\newcommand\physrep{Phys.~Rep.}%
          % Physics Reports
\newcommand\physscr{Phys.~Scr}%
          % Physica Scripta
\newcommand\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\newcommand\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

